Topological quantum field theories and homotopy cobordisms

We construct a category $\mathrm{HomCob}$ whose objects are {\it homotopically 1-finitely generated} topological spaces, and whose morphisms are {\it cofibrant cospans}. Given a manifold submanifold pair $(M,A)$, we prove that there exists functors into $\mathrm{HomCob}$ from the full subgroupoid of the mapping class groupoid $\mathrm{MCG}_{M}^{A}$, and from the full subgroupoid of the motion groupoid $\mathrm{Mot}_{M}^{A}$, whose objects are homotopically 1-finitely generated. We also construct a family of functors $\mathsf{Z}_G\colon \mathrm{HomCob}\to \mathbf{Vect}$, one for each finite group $G$. These generalise topological quantum field theories previously constructed by Yetter, and an untwisted version of Dijkgraaf-Witten. Given a space $X$, we prove that $\mathsf{Z}_G(X)$ can be expressed as the $\mathbb{C}$-vector space with basis natural transformation classes of maps $\{\pi(X,X_0)\to G\} $ for some finite representative set of points $X_0\subset X$, demonstrating that $\mathsf{Z}_G$ is explicitly calculable.

==> tex/macros-magmoids.tex <==
\newcommand{\graphh}[2]{\xymatrix{#1 \ar@{=>}[r]^s_t & #2}}
\newcommand{\graphhh}[2]{\xymatrix{#1 \ar@<-.5ex>[r]_t \ar@<.5ex>[r]^s & #2}} % graph G-X
\newcommand{\mM}{{\mathsf M}}
\newcommand{\cC}{{\mathsf C}}
\newcommand{\MAG}{{\mathbf{Mag}}}

\newcommand{\rR}{{\mathsf R}}

\newcommand{\tTopo}{{\mathsf{Top}}}  %% magmoid of spaces and maps
\newcommand{\sSet}{{\mathsf{Set}}}  %% magmoid of sets and maps
\newcommand{\vVectk}{{\mathsf{Vect}_\mathbbm{k}}}  %% magmoid of vector spaces and linear maps
\newcommand{\vVectC}{{\mathsf{Vect}_\mathbbm{C}}}
